Ambient FSK Backscatter Communications using LTE Cell Specific Reference Signals

Long Term Evolution (LTE) signal is ubiquitously present in electromagnetic (EM) background environment, which make it an attractive signal source for the ambient backscatter communications (AmBC). In this paper, we propose a system, in which a backscatter device (BD) introduces artificial Doppler shift to the channel which is larger than the natural Doppler but still small enough such that it can be tracked by the channel estimator at the User Equipment (UE). Channel estimation is done using the downlink cell specific reference signals (CRS) that are present regardless the UE being attached to the network or not. FSK was selected due to its robust operation in a fading channel. We describe the whole AmBC system, use two receivers. Finally, numerical simulations and measurements are provided to validate the proposed FSK AmBC performance.

==> Complex_case.tex <==
\section{Cepstral processing II - Complex cepstrum}
Let us factor $\hat{H}[n;m]$ as follows 
\begin{eqnarray}
\hat{H}_p[n;m] &=& a_{p,0} e^{-i(\omega_n \tau_{p,0} + \phi_{p,0})} \nonumber\\
& &\times \left( 1+ \frac{a_{p,1}}{a_{p_0}} e^{-i(\omega_n \Delta \tau_{p,1}+\Delta\phi_{p,1})} x_1[m] \right. \nonumber\\
& &\left.+ \sum_{k=2}^K \frac{a_{p,k}}{a_{p,0}} e^{-i(\omega_n\tau_{p,k}+\Delta\phi_{p,k})}x_k[m]\right)\nonumber\\
& &\times \left(1+\frac{z_{p}[n;m]}{\hat{H}_p[n,m]}\right)
\end{eqnarray}
Now taking the logarithm yields 
\begin{eqnarray}\label{eq:lnH_n}
\ln\hat{H}_p[n;m] &\approx& \ln a_0 -i(\omega_n \tau_{p,0} + \phi_{p,0})\nonumber \\
& &+\frac{a_{p,1}}{a_{p_0}} e^{-i(\omega_n \Delta \tau_{p,1}+\Delta\phi_{p,1})} x_1[m] \nonumber\\
& &+\sum_{k=2}^K \frac{a_{p,k}}{a_{p,0}} e^{-i(\omega_n\tau_{p,k}+\Delta\phi_{p,k})}x_k[m] \nonumber\\
& &+\Xi_p[n;m]
\end{eqnarray}
where 
$$
\Xi_p[n;m]=\ln\left(1+\frac{z_{p}[n;m]}{H_p[n,m]}\right) \triangleq \Xi_p^{I}[m,n] +i \Xi_p^{Q}[m,n]
$$
denotes the log-transformed complex noise. If the SNR $\gamma_p[n;m]\triangleq\frac{|H_p[n;m|^2}{\sigma_z^2}>0$, then by Taylor expansion, we find that 
$$
\mathbb{E}\{\Xi_p[n;m]\}=0
$$
and

\begin{eqnarray*}
\mathbb{E}\{|\Xi_p[n;m]|^2\}=\frac{1}{\gamma_p[n;m]}+ \frac{1}{2}\frac{1}{\gamma_p^2[n;m]}+\frac{2}{3}\frac{1}{\gamma_p^3[n;m]}\\
+\frac{3}{2}\frac{1}{\gamma_p^4[n;m]}+\frac{24}{5}\frac{1}{\gamma_p^5[n;m]}+... \triangleq\sigma_{\Xi,p}^2[n;m]
\end{eqnarray*}
In high SNR, $\mathbb{E}\{|\Xi_p[n;m]|^2\}\approx\frac{1}{\gamma_p[n;m]}$.


The real part 
\begin{eqnarray}
\mathrm{Re}\ln\hat{H}_p[n;m] &\approx& \ln a_0 \nonumber \\
& &+\frac{a_{p,1}}{a_{p_0}} \cos(\omega_n \Delta \tau_{p,1}+\Delta\phi_{p,1}) x_1[m] \nonumber\\
& &+\sum_{k=2}^K \frac{a_{p,k}}{a_{p,0}} \cos(\omega_n\tau_{p,k}+\Delta\phi_{p,k})x_k[m] \nonumber\\
& &+\Xi_p^{(I)}[n;m] \triangleq L_p^I[n;m]
\end{eqnarray}
has a complex bias $\mathbb{E}\{\Xi_p^{(I)}\}+\ln a_0$ that we can remove by using mean removal. Let us define
\begin{equation}
    Y_p^I[q,m]= L_p^I[m;n]- \frac{1}{N}\sum_{n=0}^{N-1} L_p^I[m;n] 
\end{equation}
The imaginary part 
\begin{eqnarray}
\mathrm{Im}\ln\hat{H}_p[n;m] &\approx& -(\omega_n \tau_{p,0} + \phi_{p,0})\nonumber \\
& &+\frac{a_{p,1}}{a_{p_0}} \sin(\omega_n \Delta \tau_{p,1}+\Delta\phi_{p,1}) x_1[m] \nonumber\\
& &+\sum_{k=2}^K \frac{a_{p,k}}{a_{p,0}} \sin(\omega_n\tau_{p,k}+\Delta\phi_{p,k})x_k[m] \nonumber\\
& &+\Xi_p^{(Q)}[n;m] \triangleq L_p^Q[n;m]
\end{eqnarray}
has a linear trend $\mathbb{E}\{\Xi_p^{(Q)}[n;m]\}-(\omega_n \tau_{p,0} + \phi_{p,0}) = \beta_{p,0} +\beta_{p,1}n $ which we must first estimate by solving a quadratic problem
$$
\min_{\beta_{p,0},\beta_{p,1}} \sum_{n=0}^{N-1}\left(L_p^I[n;m]-\beta_{p,0} -\beta_{p,1}n\right)^2
$$
Let us define trend removed signal
\begin{equation}
    Y_p^Q[q,m]= L_p^Q[m;n]- \beta_{p,0}-\beta_{p,1}n
\end{equation}
Now the direct path removed complex signal can be written as
$$
Y_{p}[n;m] = Y_{p}^I[n;m]+iY_{p}^Q[n;m] 
$$

Let $\varphi_{p,k}=2\pi f_0 + \phi_{p,k}-\phi_{p,0}$. Assume that $\Delta f \Delta \tau_k N = q_k$ is an integer. Inverse Discrete Fourier Transform (IDFT) of $Y_{p}[n;m]$, yields
\begin{eqnarray}\label{eq:complex_y}
y_{p}[q;m] &=& \frac{a_{p,1}}{a_{p,0}}e^{i\varphi_{p,1}}\delta(q-q_1)\nonumber\\
& & +  \sum_{k=2}^K \frac{a_{p,k}}{a_{p,0}}e^{i\varphi_{p,k}}\delta(q-q_k) \nonumber\\
& & + \xi_{p}[q;m]
\end{eqnarray}
where the noise term
$$
\xi_{p}[q;m] =\frac{1}{N} \sum_{n=0}^{N-1} \Xi_p[n;m] e^{i\frac{2\pi}{N}qn}
$$
becomes approximately complex normal Gaussian random variable for large $N$:
$$
\xi_{p}[q;m] \sim \mathcal{C}{N} \left(0,\sigma_{\xi,p}^2[q;m]\right)
$$
where 
$$
\sigma_{\xi,p}^2[q;m]= \frac{1}{N^2}\sum_{n=0}^{N-1}\sigma_{\Xi,p}^2[n;m] =\frac{1}{N\rho_{p}[m]}
$$
where
$$
\rho_{p}[m]= \left(\frac{1}{N}\sum_{n=0}^{N-1}\sigma_{\Xi,p}^2[n;m]\right)^{-1}
$$
denotes effective SNR of the channel. 

If the backscatter devices are favourably spaced from each other such that $q_k\neq q_l$, for $k\neq l$, then the SNR seen by the backscatter devices after the complex cepstral processing is 
$$
\Gamma_k[m]=N\frac{a_{p,k}^2}{a_{p,0}^2}\rho_p[m]
$$
This is factor-2 larger than in the case of real (power) cepstrum.
